BRPO: Batch Residual Policy Optimization

In batch reinforcement learning (RL), one often constrains a learned policy to be close to the behavior (data-generating) policy, e.g., by constraining the learned action distribution to differ from the behavior policy by some maximum degree that is the same at each state. This can cause batch RL to be overly conservative, unable to exploit large policy changes at frequently-visited, high-confidence states without risking poor performance at sparsely-visited states. To remedy this, we propose residual policies, where the allowable deviation of the learned policy is state-action-dependent. We derive a new for RL method, BRPO, which learns both the policy and allowable deviation that jointly maximize a lower bound on policy performance. We show that BRPO achieves the state-of-the-art performance in a number of tasks.

==> experiments.tex <==

%%% CEB: moved the table earlier in Section 5 so it would end up on page 6, not page 7 of PDF

% \begin{table*}[th!]
% \scriptsize
% \setlength\tabcolsep{1.5pt}
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Environment-$\varepsilon$ & DQN & SARSA & BRPO-C & BRPO & Behavior Cloning & BCQ \\
% \hline
% Acrobot-0.15 &
% \tb{-92.6} $\pm$ 62.2 & -117.1 $\pm$ 114.2 & -95.4 $\pm$ 88.7 & -93.0 $\pm$ 83.3 & -189.6 $\pm$ 19.6 & \tb{-84.5} $\pm$ 9.3
% \\ Acrobot-0.25 &
% \tb{-86.9} $\pm$ 70.0 & -98.8 $\pm$ 103.0 & -91.7 $\pm$ 114.4 & -89.1 $\pm$ 101.6 & -198.5 $\pm$ 22.5 & \tb{-83.7} $\pm$ 9.0
% \\ Acrobot-0.50 &
% \tb{-84.9} $\pm$ 58.3 & -87.9 $\pm$ 70.6 & -86.7 $\pm$ 87.1 & -87.2 $\pm$ 118.6 & -278.1 $\pm$ 28.3 & \tb{-82.9} $\pm$ 8.5
% \\ Acrobot-0.75 &
% \tb{-82.8} $\pm$ 59.9 & -96.8 $\pm$ 91.4 & -89.7 $\pm$ 122.2 & \tb{-86.9} $\pm$ 143.2 & -416.1 $\pm$ 29.8 & -134.5 $\pm$ 91.1
% \\ Acrobot-1.00 &
% -132.9 $\pm$ 152.7 & -126.8 $\pm$ 147.6 & \tb{-112.3} $\pm$ 155.1 & \tb{-109.5} $\pm$ 143.1 & -496.5 $\pm$ 4.9 & -229.7 $\pm$ 123.9\\
% \hline
% CartPole-0.15 &
% 9.4 $\pm$ 0.3 & 95.1 $\pm$ 76.2 & 92.0 $\pm$ 77.9 & \tb{161.8} $\pm$ 73.7 & 62.7 $\pm$ 15.0 & \tb{165.8} $\pm$ 28.4
% \\ CartPole-0.25 &
% 9.5 $\pm$ 0.3 & 194.1 $\pm$ 64.9 & \tb{200.0} $\pm$ 68.4 & \tb{199.8} $\pm$ 70.2 & 59.1 $\pm$ 13.0 & 175.2 $\pm$ 39.9
% \\ CartPole-0.50 &
% 47.5 $\pm$ 76.3 & \tb{200.0} $\pm$ 1.7 & 200.0 $\pm$ 26.5 & \tb{200.0} $\pm$ 0.8 & 40.9 $\pm$ 9.0 & 173.8 $\pm$ 42.7
% \\ CartPole-0.75 &
% 200.0 $\pm$ 13.4 & \tb{200.0} $\pm$ 0.0 & 198.7 $\pm$ 26.2 & \tb{200.0} $\pm$ 1.6 & 30.0 $\pm$ 6.0 & 161.3 $\pm$ 45.9
% \\ CartPole-1.00 &
% 185.5 $\pm$ 12.5 & \tb{200.0} $\pm$ 8.1 & \tb{200.0} $\pm$ 5.5 & 193.9 $\pm$ 31.1 & 23.7 $\pm$ 4.2 & 88.2 $\pm$ 49.3\\
% \hline
% LunarLander-0.15 &
% -133.6 $\pm$ 118.9 & 21.6 $\pm$ 127.2 & 29.8 $\pm$ 114.7 & \tb{130.0} $\pm$ 82.6 & 42.4 $\pm$ 27.3 & \tb{146.5} $\pm$ 55.4 \\
% LunarLander-0.25 &
% -73.0 $\pm$ 171.3 & -29.8 $\pm$ 97.7 & \tb{235.1} $\pm$ 69.8 & \tb{234.7} $\pm$ 132.7 & 15.4 $\pm$ 26.9 & 146.5 $\pm$ 63.8 \\
% LunarLander-0.50 &
% 159.5 $\pm$ 139.7 & 61.9 $\pm$ 87.7 & \tb{233.7} $\pm$ 80.7 & \tb{224.4} $\pm$ 84.8 & -54.5 $\pm$ 23.1 & 172.0 $\pm$ 67.0 \\
% LunarLander-0.75 &
% -8.0 $\pm$ 121.7 & -67.0 $\pm$ 106.5 & \tb{127.6} $\pm$ 167.5 & \tb{186.4} $\pm$ 81.9 & -102.6 $\pm$ 25.1 & -8.2 $\pm$ 160.3 \\
% LunarLander-1.00 &
% 5.7 $\pm$ 131.7 & \tb{41.8} $\pm$ 113.6 & 37.1 $\pm$ 91.3 & \tb{108.7} $\pm$ 90.7 & -166.3 $\pm$ 36.0 & -60.2 $\pm$ 93.9 \\
% \hline
% \end{tabular}
% \vspace{-1mm}
% \caption{The mean and st.\ dev. of average returns with the best hyper-parameter configuration (the top 2 performances boldfaced). Full training curves are given in Fig.~\ref{fig:exp1_best_mean} in Appendix~\ref{additional_plots} along with the behavior policies. For \BCRPO{}-C, a parameter sweep was used to find a single constant ($0.5)$ that works well across all dataset.}
% \label{table:exp1_best_mean}
% \end{table*}



To illustrate the effectiveness of \BCRPO{}, we compare it with several state-of-the-art batch RL methods on the following discrete-action OpenAI Gym tasks~\citep{openaigym} : \cart{} (CP), \luna{} (LL), and \acro{} (AB).
For each task, five trajectory datasets that represent different batch training scenarios are generated to evaluate the trade-offs of each method.

We compare \BCRPO{} with four baseline methods, a batch version of DQN \citep{mnih2013playing} SARSA \citep{sutton2018reinforcement}, Behavior Cloning (BC) \citep{kober2010imitation}, and BCQ \citep{fujimoto2018off}. \footnote{For algorithms originally designed for online setting, we modify the data collection scheme to sample from batch data.}
We also consider a constant variant \BCRPO{}-C that treats the confidence as a tunable parameter, which is similar to CPI~\citep{kakade2002approximately}.

% this \BCRPO{} variant allows assessment on how the policy quality is affected by various confidence measurement that reflects the correlation between learning and the visiting frequency of the batch data.

% (ii) Variance (V), which is a heuristic that is the ratio between the variance of the ensemble optimal Q-functions and that of the ensemble SARSA Q-functions, (iii) Occupation Measure (OM), which is another heuristic that measures the ratio of state-action visitation frequency between the candidate policy and the behavior policy, 

% Note that \BCRPO{}-C counterpart is similar to CPI \cite{kakade2002approximately} and \BCRPO{}-OM
% reflects some aspects of SPIBB \cite{laroche2017safe}. 
% These \BCRPO{} variants allow assessment on how the policy quality is affected by various ways of measuring confidence that reflects the correlation between learning and the visiting frequency of the batch data.
 
% We evaluate \BCRPO{} on the aforementioned Gym tasks, whose action space is discrete. 
% The behavior policy for each environment is trained via standard DQN \citep{mnih2013playing}. Similar to other batch RL experiments (e.g., BCQ~\citep{fujimoto2018off}) we terminate the behavior policy training when its performance reaches $\sim75\%$ of the optimal performance.

The behavior policy of each environment is trained via standard DQN \citep{mnih2013playing} till it reaches $\sim75\%$ of the optimal performance, similar to other batch RL experiments (e.g., BCQ~\citep{fujimoto2018off}).
To understand how exploration and behavior policy optimality affects learning, we generate five data sets for each task (environment) by injecting different random exploration to the same behavior policy. Specifically, we added $\varepsilon$-greedy exploration to the behavior policy for $\varepsilon = 1$ (fully random), $0.75$, $0.5$, $0.25$, and $0.15$ to generate $1$ million transitions  each for batch RL training.

For fair comparisons, all models use the same architectures for the same environment. Details on network architectures and hyper-parameters are described in the appendix of the extended version. While training is entirely done offline with the batch data, policy performance is evaluated online in the simulator at every $1000$ training iterations.
Each measurement is an average return over $5$ random seeds.
To smooth the learning curves, data points are averaged over a sliding window of size $3$.

% Results
Table~\ref{table:exp1_best_mean} shows the average return of \BCRPO{} and other batch RL baselines under the best hyper-parameter configurations. Under the full-exploration ($\varepsilon=1$) batch setting, value-based methods, such as DQN and SARSA, have the best performance. Methods that mimic or follow the behavior policy closely like BCQ, \footnote{This observation was first discovered by \citet{kumar2019stabilizing}, in which the BEAR algorithm also keeps
the learned and behavior policies close to each other by regularizing their discrepancy measures. Since these algorithms fundamentally have similar essence, for simplicity we decide to only focus on comparing with BCQ.} are among the worst performing ones. These phenomena are totally reverse in the low-exploration cases, i.e., $\varepsilon\in\{0.15, 0.25\}$, where BCQ have good performance while DQN and SARSA struggle to learn.

These observations corroborate with the intuitions that (i) DQN and SARSA require a good amount of exploration to learn effectively, or otherwise, may have instability issues due to their vulnerability to out-of-distribution errors; (ii) BCQ improves the performance of the behavior policy locally but are quite conservative, where the final policies don't deviate too much from $\pibehavior$. To achieve the best in both scenarios, \BCRPO{} takes account of the statistics of each $(s, a)$ pair in data during training and is able to achieve good performance in almost all scenarios, collectively outperforming other baselines. 
On the other hand, \BCRPO{}-C, a simplified version of \BCRPO{} with a constant confidence parameter, also exhibits decent performance and robustness to different degree of exploration. However, finding the optimal confidence requires extensive hyper-parameter search, which can be rather computationally expensive.

In general, stable performance and robustness across various scenarios make \BCRPO{} a practical choice of batch RL algorithm, especially in many real-world problems it is difficult to estimate the amount of exploration in data generation prior to training, when
one only has access to the batch data.

% Among the four different confidence models, the constant-based confidence requires extensive hyper-parameter tuning, whereas both the variance-based and the occupation-measure-based counterparts involve complex value function learning---the former requires training an ensemble of Q-functions to estimate the variance~\citep{kumar2019stabilizing}, while the latter requires learning two dual value functions. In comparison, our proposed method, which formulates $\lambda$ learning as a QP (plus distribution matching), provide additional computational benefits. Performance-wise, Res-OPT is among the best ones in all the experiments, while the results of Res-V and Res-C tend to have higher variance. Worth-noting that all \BCRPO{} methods outperform the behavior performance after learning stabilizes, though due to function approximation errors their initial performance may be much lower (see Figure~\ref{fig:exp1_best_mean} in Appendix for details). 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%     \item How does policy mixing compare to each of the behavior and residual policy component
%     \item How is our method compared to other existing RL algorithms (batch-RL, off-policy, etc.)
% \end{itemize}

% The behavior agent was trained via DQN \cite{dqn-atari} for the three tasks, using the same set of hyperparameters.
% Similar to BCQ and BEAR, we select the model checkpoint when the agent first reaches a normalized performance of around $40\%-60\%$ for each game, where the normalized performance is computed by normalizing the average return with respect to the performance of random policy and optimal policy.



% We designed our experiments to answer the following questions and to verify our method:
% \cutitemizeup
% \begin{itemize}
% \tightlist
%     \item How does the stochasticity or \emph{exploration} of the behavior policy affect the learning
%     \item How does the behavior policy performance affects our final policy, especially if there is trade-off with exploration
%     \item How does policy mixing compare to each of the behavior and residual policy component
%     \item How is our method compared to other existing RL algorithms (batch-RL, off-policy, etc.)
% \end{itemize}

% \subsection{Experiment setting}
% We evaluated the proposed method on three Open-AI gym~\cite{openaigym} tasks for discrete action: \cart{}, \acro{}, and \luna{}. 
% Our method \BCRPO{} was compared with existing  batch-RL methods, like BEAR~\cite{kumar2019stabilizing} and DBCQ~\cite{jaques2019way}. For each set of transition data generated by some behavior policy, we train each method using the same architecture to have a fair comparison.


% The behavior agent was trained via DQN \cite{dqn-atari} for the three tasks, using the same set of hyperparameters.
% Similar to BCQ and BEAR, we select the model checkpoint when the agent first reaches a normalized performance of around $40\%-60\%$ for each game, where the normalized performance is computed by normalizing the average return with respect to the performance of random policy and optimal policy.

% From the $Q$-function corresponding to the model checkpoint, we created several variants of behavior policies with different optimality and exploration trade-offs. In particular, we applied $\varepsilon$-Greedy and Boltzmann policy wrapper on top of the same $Q$-function with different $\varepsilon$ and temperature $\tau$ for generating trajectory data. For each behavior policy variant, we generated offline data set consisting of 1 million transitions for batch training. We report the result averaged over 5 random seeds. See supplemental material for more details.




% % Controlling exploration in data generation (Figure 1)

% \subsection{Result}
% % Ours V.S. others
% We compared our \BCRPO{} agent against batch-RL methods (e.g DBCQ, BEAR), DQN, and behavior policy in Figure~\ref{fig:sota}. The DQN agent fails to outperform the behavior policy due to the \emph{extrapolation error}~\cite{fujimoto2018off}, even though it was trained for more number of steps with larger replay buffer. The DBCQ method performs worse than DQN as it is overly restrictive, which becomes more severe in discrete action domain, as also shown in~\citet{jaques2019way}. BEAR outperforms the behavior policy on two of the three tasks. Our \BCRPO{} method was able to improves over the behavior policy on all the tasks with larger margin. 
% TODO: check if we claim this in the method


% \subsection{Analysis}
% In this section, we evaluate the advantage of the learned confidence function $\lambda(s, a)$ over the constant confidence and the ensemble variance-based confidence~\cite{kumar2019stabilizing}. The result shows that....



% \iffalse
% \begin{comment}
% % Ablation
% \subsection{Analysis}
% In this section, we conduct an ablation study to evaluate how much each component contributes to the final performance. The result is summarized in Figure~\ref{fig:ablation}. We first compared \BCRPO{} with expected SARSA and soft-Q learning method as the update rule of \BCRPO{} is a weighted sum of expected SARSA and soft-Q. The result shows that our \BCRPO{} consistently outperforms expected SARSA and soft-Q method. In fact, we claim that \BCRPO{} takes advantage of both agents. Figure~\ref{fig:analysis} shows that expected SARSA suffers less from the overestimation problem of Q-value~\cite{} compared to soft-Q method.
% \end{comment}
% \fi

==> extra/rebuttal.tex <==
\begin{table*}[th!]
\scriptsize
\setlength\tabcolsep{1.5pt}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Environment-$\varepsilon$ & DQN & SARSA & BRPO (const) & BRPO (opt) & Behavior Cloning & BCQ \\
\hline
Acrobot-0.15 &
\tb{-92.6} $\pm$ 62.2 & -117.1 $\pm$ 114.2 & -95.4 $\pm$ 88.7 & -93.0 $\pm$ 83.3 & -189.6 $\pm$ 19.6 & \tb{-84.5} $\pm$ 9.3
\\ Acrobot-0.25 &
\tb{-86.9} $\pm$ 70.0 & -98.8 $\pm$ 103.0 & -91.7 $\pm$ 114.4 & -89.1 $\pm$ 101.6 & -198.5 $\pm$ 22.5 & \tb{-83.7} $\pm$ 9.0
\\ Acrobot-0.50 &
\tb{-84.9} $\pm$ 58.3 & -87.9 $\pm$ 70.6 & -86.7 $\pm$ 87.1 & -87.2 $\pm$ 118.6 & -278.1 $\pm$ 28.3 & \tb{-82.9} $\pm$ 8.5
\\ Acrobot-0.75 &
\tb{-82.8} $\pm$ 59.9 & -96.8 $\pm$ 91.4 & -89.7 $\pm$ 122.2 & \tb{-86.9} $\pm$ 143.2 & -416.1 $\pm$ 29.8 & -134.5 $\pm$ 91.1
\\ Acrobot-1.00 &
-132.9 $\pm$ 152.7 & -126.8 $\pm$ 147.6 & \tb{-112.3} $\pm$ 155.1 & \tb{-109.5} $\pm$ 143.1 & -496.5 $\pm$ 4.9 & -229.7 $\pm$ 123.9\\
\hline
CartPole-0.15 &
9.4 $\pm$ 0.3 & 95.1 $\pm$ 76.2 & 92.0 $\pm$ 77.9 & \tb{161.8} $\pm$ 73.7 & 62.7 $\pm$ 15.0 & \tb{165.8} $\pm$ 28.4
\\ CartPole-0.25 &
9.5 $\pm$ 0.3 & 194.1 $\pm$ 64.9 & \tb{200.0} $\pm$ 68.4 & \tb{199.8} $\pm$ 70.2 & 59.1 $\pm$ 13.0 & 175.2 $\pm$ 39.9
\\ CartPole-0.50 &
47.5 $\pm$ 76.3 & \tb{200.0} $\pm$ 1.7 & 200.0 $\pm$ 26.5 & \tb{200.0} $\pm$ 0.8 & 40.9 $\pm$ 9.0 & 173.8 $\pm$ 42.7
\\ CartPole-0.75 &
200.0 $\pm$ 13.4 & \tb{200.0} $\pm$ 0.0 & 198.7 $\pm$ 26.2 & \tb{200.0} $\pm$ 1.6 & 30.0 $\pm$ 6.0 & 161.3 $\pm$ 45.9
\\ CartPole-1.00 &
185.5 $\pm$ 12.5 & \tb{200.0} $\pm$ 8.1 & \tb{200.0} $\pm$ 5.5 & 193.9 $\pm$ 31.1 & 23.7 $\pm$ 4.2 & 88.2 $\pm$ 49.3\\
\hline
LunarLander-0.15 &
-133.6 $\pm$ 118.9 & 21.6 $\pm$ 127.2 & 29.8 $\pm$ 114.7 & \tb{130.0} $\pm$ 82.6 & 42.4 $\pm$ 27.3 & \tb{146.5} $\pm$ 55.4 \\
LunarLander-0.25 &
-73.0 $\pm$ 171.3 & -29.8 $\pm$ 97.7 & \tb{235.1} $\pm$ 69.8 & \tb{234.7} $\pm$ 132.7 & 15.4 $\pm$ 26.9 & 146.5 $\pm$ 63.8 \\
LunarLander-0.50 &
159.5 $\pm$ 139.7 & 61.9 $\pm$ 87.7 & \tb{233.7} $\pm$ 80.7 & \tb{224.4} $\pm$ 84.8 & -54.5 $\pm$ 23.1 & 172.0 $\pm$ 67.0 \\
LunarLander-0.75 &
-8.0 $\pm$ 121.7 & -67.0 $\pm$ 106.5 & \tb{127.6} $\pm$ 167.5 & \tb{186.4} $\pm$ 81.9 & -102.6 $\pm$ 25.1 & -8.2 $\pm$ 160.3 \\
LunarLander-1.00 &
5.7 $\pm$ 131.7 & \tb{41.8} $\pm$ 113.6 & 37.1 $\pm$ 91.3 & \tb{108.7} $\pm$ 90.7 & -166.3 $\pm$ 36.0 & -60.2 $\pm$ 93.9 \\
\hline
\end{tabular}
\vspace{-0.1in}
\caption*{Table}
%BRPO (full) is the full algorithm with learned $\lambda$ proposed by this paper. BRPO-Const substitutes the learned $\lambda$ with a fixed 0.5 constant, which is found to perform well across all games.}
\label{table:exp1_rebuttal/best_mean}
\vspace{-0.1in}
\end{table*}



\label{additional_plots}
\begin{figure*}[!ht]
    \vspace*{-3pt}
    \centering
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/Acrobot_0_15.pdf}\,
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/Acrobot_0_25.pdf}\,
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/Acrobot_0_5.pdf}\,
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/Acrobot_0_75.pdf}\,
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/Acrobot_1_0.pdf}\\
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/CartPole_0_15.pdf}\,
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/CartPole_0_25.pdf}\,
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/CartPole_0_5.pdf}\,
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/CartPole_0_75.pdf}\,
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/CartPole_1_0.pdf}\\
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/LunarLander_0_15.pdf}\,
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/LunarLander_0_25.pdf}\,
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/LunarLander_0_5.pdf}\,
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/LunarLander_0_75.pdf}\,
    \includegraphics[draft=false,width=0.19\linewidth]{./figs/rebuttal/best_mean/LunarLander_1_0.pdf}%
    \vspace{-8pt}
    \caption*{Figure}
    %\caption{%
    %    The mean $\pm$ standard error (shadowed area) of mean returns.
    %    Row 1: A-0.15, A-0.25, A-0.5 A-0.75, A-1.0
    %    Row 2: CP-0.15, CP-0.25, CP-0.5 CP-0.75, CP-1.0
    %    Row 3: LL-0.15, LL-0.25, LL-0.5 LL-0.75, LL-1.0
    %    (A: Acrobot, CP: CartPole, LL: LunarLander)
    %}
    \label{fig:exp1_rebuttal/best_mean}
    \vspace{-7pt}
\end{figure*}

==> problem.tex <==
%!TEX root = main.tex
 
Policy-based methods \citep{ddpg, td3, sac} have been widely-used to handle continuous actions in RL.
However, they suffer from several well-known difficulties, e.g., (i) modeling high-dimensional action distributions, (ii) handling action constraints, and (iii) data-inefficiency.
Motivated by earlier work on value-based RL methods, such as QT-Opt \citep{kalashnikov2018qt} and actor-expert \citep{Lim18}, we
propose \emph{Continuous Action Q-learning (CAQL)}, a general framework for continuous-action value-based RL, in which the Q-function is parameterized by a NN (Eq.~\ref{eq:nnet}).  One novelty of CAQL is the
formulation of the ``max-Q'' problem, i.e., the inner maximization in (\ref{eq:dqn_l2}) and (\ref{q_problem_unc_2_saa_theta_target}), as a mixed-integer programming (MIP). 

The benefit of the MIP formulation is that it guarantees that we find the optimal action (and its true bootstrapped Q-value)
when computing target labels (and at inference time). We show empirically that this can induce
better performance, especially when the Q-network has sufficient representation power.
Moreover, since MIP can readily model linear and combinatorial constraints, 
it offers considerable flexibility when incorporating complex action constraints in RL.
That said, finding the optimal Q-label (e.g., with MIP) is computationally intensive. To alleviate this, we develop several approximation methods to systematically reduce the computational demands of the inner maximization.
In Sec.~\ref{sec:action_fun}, we introduce the \emph{action function} to approximate the $\argmax$-policy at inference time, and in Sec.~\ref{sec:dfc} we propose three techniques, \emph{dynamic tolerance}, \emph{dual filtering}, and \emph{clustering}, to speed up max-Q computation during training.


%Policy-based deep RL approaches (\cite{ddpg}, \cite{td3}, \cite{sac}) have long been studied for continuous action problems.
%They directly learn a parameterized policy (e.g., a Gaussian distribution over actions conditioned on some state representations) to maximize the expected return.
%However, such an idea is not well suited for certain applications.
%For example, in applications such as recommendation systems, where the action (output items) is a high-dimensional continuous item feature, it is unclear whether the policy can be modeled by common distributions.
%Additionally, in practice, domain experts often want to guarantee some constraints for the action variables.
%For example, they might want to restrict the action variables in a small range for a safety reason.
%In general, it is also non-trivial to define policy parameterizations that handle action constraints.
%On the other hand, value-based algorithms are well suited for handling the aforementioned situations and has several advantages over current policy search methods.
%
%Continuous Action Q-Learning (CaQL) provides a general framework to handle continuous action variables in Q-learning.
%Different from the policy-based deep RL algorithms, CaQL directly learns the optimal Q-function.
%CaQL employs various novel ideas, in particular, we show that for a specific class of Q-function networks, solving for the optimal actions can be posed as a mixed-integer programming (MIP) problem.
%The benefit of using MIP for Q-learning is that it can find a provably optimal action for the inner maximization of Q-learning (i.e., $\arg\max_a Q_\theta\ (x, a)$).
%% In addition, if constraints are linear in the action variables, such constraints can be easily formulated in the MIP formulation, and MIP can compute the optimal action that meets the constraints.
%In addition, since MIP can model a wide range of combinatorial optimization problems (e.g.\ routing, scheduling, packing), it provides the flexibility to model complex combinatorial action spaces.
%However, MIP is compute-intensive compared to various approximate optimization methods.
%We propose novel ideas for speeding up the computation of the Q-learning inner maximization for both training and serving.
%Action function is proposed to speed up serving, and we propose three techniques, namely (i) dynamic tolerance, (ii) dual filtering, (iii) clustering to speed up training, which will be explained in detail in Section~\ref{sec:dfc}.

\vspace{-0.1in}
\subsection{Plug-N-Play Max-Q Optimizers}\label{sec:max_q_solver}
\vspace{-0.1in}

 In this section, we illustrate how the max-Q problem, with the Q-function represented by a ReLU network, can be formulated as a MIP, which can be solved using off-the-shelf optimization packages (e.g., SCIP \citep{GleixnerEtal2018OO}, CPLEX \citep{cplex2009v12}, Gurobi \citep{gurobi2015gurobi}). In addition, we detail how approximate optimizers, specifically,
gradient ascent (GA) and the cross-entropy method (CEM), can trade optimality for speed in max-Q computation within CAQL.
% While the general CAQL framework is flexible to adopt any of the aforementioned methods, in experiments we show that when 
% the Q-function has sufficient representation power, then CaQL that uses optimal Bellman residual has better performance than that with CEM or GA.


% The inner maximization of Q-learning (i.e., $\arg\max_a Q_\theta\ (x, a)$), where the Q-function is approximated by a multilayer perceptron neural network, can be exactly solved by Mixed-Integer Programming (MIP) or can be approximately solved by various optimization algorithms such as Gradient Ascent or Cross-Entropy Method (CEM). In the CaQL framework, any optimization method that can handle continuous variables can be easily plugged in and out depending on the action variable dimension, neural network complexity, and the trade-off between accuracy and speed.

\vspace{-0.1in}
\paragraph{Mixed-Integer Programming (MIP)}{
A trained feed-forward ReLU network can be modeled as a MIP by formulating the nonlinear activation function at each neuron with binary constraints. Specifically, for a ReLU with pre-activation function of form $z = \max\{0, w^\top x + b\}$, where $x \in [\ell, u]$ is a $d$-dimensional bounded input, $w \in \mathbb{R}^d$, $b \in \mathbb{R}$, and $\ell, u \in \mathbb{R}^d$ are the weights, bias and lower-upper bounds respectively, consider the following set with a binary variable $\zeta$ indicating whether the ReLU is active or not:

\vspace{-0.125in}
\begin{align*}
    R(w,b, \ell,u) = \left\{(x, z, \zeta)\ \Big|\ \begin{array}{c}
    z \geq w^\top x + b,\ z \geq 0,\ z \leq w^\top x + b - M^- (1-\zeta),\ z \leq M^+ \zeta,\\[0.25em]
    (x, z, \zeta) \in [\ell, u] \times \mathbb{R} \times \{0, 1\}
    \end{array}
    \right\}.
\end{align*}
\vspace{-0.1in}

In this formulation, both $M^+ = \max_{x \in [\ell,u]} w^\top x + b$ and $M^- = \min_{x \in [\ell,u]} w^\top x + b$ can be computed in linear time in $d$. We assume $M^+ > 0$ and $M^- < 0$, otherwise the function can be replaced by $z = 0$ or $z = w^\top x + b$. These constraints ensure that $z$ is the output of the ReLU: If $\zeta = 0$, then they are reduced to $z = 0 \geq w^\top x + b$, and if $\zeta = 1$, then they become $z = w^\top x + b \geq 0$. 

This can be extended to the ReLU network in (\ref{eq:nnet}) by \emph{chaining} copies of intermediate ReLU formulations. More precisely, if the ReLU Q-network has $m_j$ neurons in layer $j\in\{2, \ldots, K\}$, for any given state $x\in X$, the max-Q problem can be reformulated as the following MIP:
\begin{align}
q^*_x=\max\quad & c^\top z_K\label{eq:mip}\\
\text{s.t.}\quad & z_1:=a \in \ball(\overline a, \Delta),\nonumber\\
&(z_{j-1}, z_{j,i}, \zeta_{j,i}) \in R(W_{j,i}, b_{j,i}, \ell_{j-1}, u_{j-1}),\,\,j\in\{ 2, \ldots, K\},\, i \in\{ 1, \ldots, m_{j}\},\nonumber
\end{align}
where $\ell_1=\overline a-\Delta, u_1=\overline a+\Delta$ are the (action) input-bound vectors. Since the output layer of the ReLU NN is linear, the MIP objective is linear as well. Here, $W_{j, i} \in \reals^{m_{j}}$ and $b_{j,i} \in \reals$ are the weights and bias of neuron $i$ in layer $j$. Furthermore, $\ell_{j},u_{j}$ are interval bounds for the outputs of the neurons in layer $j$ for $j \geq 2$, and computing them can be done via interval arithmetic or other propagation methods \citep{weng2018towards} from the initial action space bounds (see Appendix \ref{appendix:derivations_dual_filtering} for details). As detailed by \citet{Anderson19}, this can be further tightened with additional constraints, and its implementation can be found in the \textit{tf.opt} package described therein. As long as these bounds are redundant, having these additional box constraints will not affect optimality. 
We emphasize that the MIP returns \emph{provably global optima}, unlike GA and CEM. Even when interrupted with stopping conditions such as a time limit, MIP often produces high-quality solutions in practice.

In theory, this MIP formulation can be solved in time exponential on the number of ReLUs and polynomial on the input size (e.g., by naively solving an LP for each binary variable assignment).
In practice however, a modern MIP solver combines many different techniques to significantly speed up this process, such as branch-and-bound, cutting planes, preprocessing techniques, and primal heuristics \citep{linderoth1999computational}.
Versions of this MIP model have been used in neural network verification~\citep{cheng2017maximum,lomuscio2017approach,bunel2018unified,dutta2018output,fischetti2018deep,Anderson19,tjeng2017evaluating} and analysis~\citep{serra2018bounding,kumar2019equivalent}, but its \emph{application to RL is novel}. While
\cite{say17} also proposed a MIP formulation to solve the planning problem with non-linear state transition dynamics model learned with a NN, it is different than ours, which solves the max-Q problem. 

}


% \paragraph{Mixed-Integer Linear Programming (MILP)}
% A trained multilayer perceptron (MLP) neural network with ReLU activations can be modeled via mixed-integer programming by formulating each individual neuron. For each ReLU of the form $z = \max\{0, w^\top x + b\}$ with a $d$-dimensional bounded input $x \in [L, U]$, where $w \in \mathbb{R}^d$, $b \in \mathbb{R}$, and $L, U \in \mathbb{R}^d$, we may add a binary variable $\zeta$ that indicates whether the ReLU is active or not, as follows:
% \begin{align*}
%     R(w,b) = \left\{(x, z, \zeta)\ \Big|\ \begin{array}{c}
%     z \geq w^\top x + b,\ z \geq 0,\ z \leq w^\top x + b - M^- (1-\zeta),\ z \leq M^+ \zeta,\\[0.25em]
%     (x, z, \zeta) \in [L, U] \times \mathbb{R} \times \{0, 1\}
%     \end{array}
%     \right\}.
% \end{align*}

% Above, $M^+ = \max_{x \in [L,U]} w^\top x + b$ and $M^- = \min_{x \in [L,U]} w^\top x + b$, which can be computed in linear time on $d$. The formulation is valid since if $z = 0$, then it collapses to $y = 0 \geq w^\top x + b$, and if $z = 1$, then it becomes $y = w^\top x + b \geq 0$. The model for the overall neural network can then be constructed by chaining copies of this formulation for each ReLU. The objective function in our case is a linear function on the last layer. More precisely, if we have a fully connected ReLU network with $m_j$ neurons in each layer $j$, the full MIP formulation is:
% \begin{align*}
% \max\ & c^\top z_K&\\
% & (z_{j-1}, z_{j,i}, \zeta_{j,i}) \in R(W_{j,i}, b_{j,i})&j = 2, \ldots, K,\ i = 1, \ldots, m_{j}\\
% & z_1 \in [\ell_1, u_1]
% \end{align*}
% where $\ell_1, u_1$ are vectors of bounds for the input of the neural network. Here, $W_{j, i} \in \reals^{m_{j}}$ and $b_{j,i} \in \reals$ are the weight vector and bias of the neuron $i$ in layer $j$. {\color{red} TODO: Fix these notations if needed.}

% Since each ReLU requires bounded inputs, bounds need to be computed via interval arithmetic or other propagation methods (e.g.~\cite{weng2018towards,singh2019abstract}) from the initial action space bounds. As detailed in~\cite{Anderson19}, this can be further tightened with additional constraints, and for our experiments we use the \textit{tf.opt} package described in that paper.

% We use a two-layer MLP for the Q-function and the action variables are the decision variables in the MIP formulation for the Q-learning inner maximization. Unlike the other methods below, MIP offers provably optimal solutions. Even when interrupted with e.g.\ a time limit, MIP often provides good quality solutions.

\vspace{-0.1in}
\paragraph{Gradient Ascent}{
GA \citep{nocedal2006numerical} is a simple first-order optimization method for finding the (local) optimum of a differentiable objective function, such as a neural network Q-function. At any state $x\in X$, given a ``seed''
% arbitrarily initialized / initial 
action $a_0$, the optimal action $\arg\max_a Q_\theta\ (x, a)$ is computed iteratively by $a_{t+1} \leftarrow a_{t} + \eta\nabla_{a}Q_{\theta}(x,a)$, 
where $\eta>0$ is a step size (either a tunable parameter or computed using back-tracking line search \citep{nocedal1998combining}). This process repeats until convergence, $\left|Q_{\theta}(x, a_{t+1}) - Q_{\theta}(x, a_{t})\right| < \epsilon$, or  a maximum iteration count is reached.}

\vspace{-0.1in}
\paragraph{Cross-Entropy Method}{
CEM \citep{Rubinstein99} is a derivative-free optimization algorithm. At any given state $x\in X$, it samples a batch of $N$ actions $\{a_i\}_{i=1}^N$ from $A$ using a fixed distribution (e.g., a Gaussian) and ranks the corresponding Q-values $\{Q_\theta(x,a_i)\}_{i=1}^N$. Using the top $K<N$ actions, it then updates the sampling distribution, e.g., using the sample mean and covariance to update the Gaussian. This is repeated until convergence or a maximum iteration count is reached.}

\vspace{-0.1in}
\subsection{Action Function}\label{sec:action_fun}
\vspace{-0.1in}
In traditional Q-learning, the policy $\pi^*$ is ``implemented'' by acting greedily w.r.t.\ the learned Q-function: 
$\pi^*(x) = \arg\max_a Q_\theta\ (x, a)$.\footnote{Some exploration strategy may be incorporated as well.}
However, computing the optimal action can be expensive in the continuous case, which may be especially problematic
at inference time (e.g.,
% at each state $x$ with this greedification step (and with the aforementioned optimization algorithms) is expensive and even intractable in situations 
when computational power is limited in, say embedded systems, or  real-time response is critical).
To mitigate the problem, we can use an \emph{action function} $\pi_{w}:X\rightarrow A$---effectively a trainable actor network---to approximate the greedy-action mapping $\pi^*$.
% w.r.t.\ $Q_\theta$. 
We train $\pi_{w}$ using training data  $B=\{(x_i,q^*_i)\}_{i=1}^{|B|}$,
% in the replay buffer,
where $q^*_i$ is the max-Q label at state $x_i$.
% computed for estimating the Bellman residual, we learn 
Action function learning is then simply a supervised regression problem: $w^* \in \arg\min_{w}\sum_{i=1}^{|B|}(q^*_i-Q_\theta(x_i, \pi_{w}(x_i)))^2$. 
This is similar to the notion of ``distilling'' an optimal policy from max-Q labels, as in actor-expert \citep{Lim18}. Unlike actor-expert---a separate stochastic policy network is jointly learned with the Q-function to maximize the likelihood with the underlying optimal policy---our method learns a state-action mapping to approximate $ \arg\max_a Q_\theta\ (x, a)$---this does not require distribution matching and is
generally more stable. The use of action function in CAQL is simply \emph{optional} to
accelerate data collection and inference. 


%Once the Q-function is learned, a policy can be obtained by acting greedily on the learned Q-function: $\pi(x) = \arg\max_a Q_\theta\ (x, a)$. However, computing the maximization for every state $x$ from a learned Q-function can be costly for certain scenarios. For example, such computation can be slow with an embedded computing device in a robot, which usually has low computational power. To overcome the problem, an action function ($\pi_w(x)$) approximated by another feed-forward neural network is learned. The action function weights are adjusted to return an action that will have a Q-value close to the maximum Q-value for a given state $x$:
%
%\vspace{-0.15in}
%\begin{equation*}
%\min_w (\max_a Q_\theta(x,a)-Q_\theta(x, \pi_w(x)))^2
%\end{equation*}
%\vspace{-0.15in}

%
%Keep in mind that, different from Actor-Expert (\cite{Lim18}), we do not use a parameterized stochastic policy. 
%Action function just approximates the optimal action for a given state to speed up the model serving, and the use of the action function in the CaQL framework is completely optional.
%If users are not sensitive to the serving latency, they can compute the optimal action at the serving time using the learned Q-function.

%The pseudocode how CaQL is trained is illustrated in Algorithm~\ref{alg:caql}.
%Note that the ideas of Section~\ref{sec:dfc} are not included in the pseudocode for concise description.

